Cellular Network Design for UAV Corridors via Data-driven High-dimensional Bayesian Optimization

We address the challenge of designing cellular networks for uncrewed aerial vehicles (UAVs) corridors through a novel data-driven approach. We assess multiple state-of-the-art high-dimensional Bayesian optimization (HD-BO) techniques to jointly optimize the cell antenna tilts and half-power beamwidth (HPBW). We find that some of these approaches achieve over 20dB gains in median SINR along UAV corridors, with negligible degradation to ground user performance. Furthermore, we explore the HD-BO's capabilities in terms of model generalization via transfer learning, where data from a previously observed scenario source is leveraged to predict the optimal solution for a new scenario target. We provide examples of scenarios where such transfer learning is successful and others where it fails. Moreover, we demonstrate that HD-BO enables multi-objective optimization, identifying optimal design trade-offs between data rates on the ground versus UAV coverage reliability. We observe that aiming to provide UAV coverage across the entire sky can lower the rates for ground users compared to setups specifically optimized for UAV corridors. Finally, we validate our approach through a case study in a real-world cellular network, where HD-BO identifies optimal and non-obvious antenna configurations that result in more than double the rates along 3D UAV corridors with negligible ground performance loss.

==> Md_backup.tex <==
\begin{comment}
\subsection{Motivation}
The establishment of robust and trustworthy connectivity is recognized as an imperative prerequisite for the flourishing of the Unmanned Aerial Vehicles (UAVs) ecosystem. This becomes particularly relevant in the context of high impact applications that UAVs will provide, ranging from goods/people delivery, traffic monitoring, weather surveillance, to search and rescue missions. Venture capitalists, having keen interest in advancing aerial mobility solutions, along with governmental associations, are proactively allocating substantial investments in the wireless telecommunications sector to fulfill the unmet requirements concerning the UAV command and control (C2) links \cite{GerGarAza2022, FotQiaDin2019}. 

Conventional terrestrial cellular base stations (BSs) are primarily designed to provide two-dimensional (2D) ground-level connectivity. Thus, the UAVs can solely be served through the upper antenna sidelobes, leading to pronounced signal instability during their motion. Furthermore, as UAVs operate above buildings, they encounter both reception and emission of line-of-sight (LoS) interfering signals emanating from the surrounding BSs. This phenomenon contributes to a deteriorating of the signal-to-interference-plus-noise ratio (SINR) of UAVs \cite{geraci2018understanding, ZenLyuZha2019}. To pursue 3D connectivity, i.e., also up in the air, re-engineering the cellular network deployed originally to serve the legacy ground users (GUEs) is needed.

The provided coverage of cellular networks are significantly influenced by the configuration of base station (BS) antennas deployed throughout the network. The direction and shape of the dominant beams, which are typically fine-tuned through adjustments to specific parameters such as the down-tilt angle, and the half-power beamwidth (HPBW) angle, hold a critical role in enhancing the received signal strength and minimizing interference. This procedure, known as cell shaping, is a periodic cell-specific optimization in response to variations in the distribution of users and other long-term network factors. The aim here is to optimize the cellular network by re-shaping the coverage area of the cell in a way that aligns with the users’ distributions. 
Such an optimization problem is nontrivial due to the reason that the settings across each cell are coupled by interference and dependent on the randomness of the users’ distribution, resulting in a multi-cell optimization problem that is non-convex and NP-hard. Another challenge stems from the conflicting nature of the two types of users (i.e., GUEs and UAVs), maximizing both performance of UAVs– which in practice means directing energy towards the sky by up-tilting the cells – and the performance of GUEs, which tends to favor cells to be down-tilted.

In an actual network deployment, the configuration of antenna parameters typically involves the utilization of site-specific radio frequency planning tools. Subsequent adjustments are often subject to trial-and-error procedures, guided by empirical field measurements gathered over a long period. Such conventional methods exhibit limitations in terms of scalability and optimality; thus, there arises a demand for practical, automated optimization methods that are well-supported by theory and utilize recent advances in data-driven models. This paper proposes the utilization of high-dimensional Bayesian Optimization (HD-BO) as a step towards addressing the mentioned limitations. 

\subsection{Prior Work}
Both academia and the mobile industry have long joined forces to pursue 3D connectivity. To provide such connectivity to UAVs without compromising the performance of existing ground users, short-term solutions are being implemented via time/frequency separation \cite{3GPP36777,NguAmoWig2018}. However, this approach can only handle a few cellular-connected UAVs; thus, becoming gradually inefficient as the number of UAVs increases, as it requires dedicated radio resources for each UAV. Other proposed solutions for ubiquitous aerial connectivity rely on dedicating infrastructure for aerial services \cite{kim2022non, mozaffari2021toward}, network densification \cite{d2020analysis,garcia2019essential,diaz2022cell}, or the integration of non-terrestrial networks; i.e., LEO satellites to complement the ground network \cite{benzaghta2022uav, geraci2022integrating}. Although those proposed solutions offer promising gains in terms of providing  connectivity to UAVs, they necessitate expensive hardware installations, signal processing improvements, and still suffer to provide ubiquitous connectivity to large constellations of aerial devices.

All of the mentioned studies are based on the premise that the UAVs will operate without limitations and that the cellular networks must ensure connectivity across all 3D space locations. Yet, similar to ground vehicles and aircrafts, the expansion of UAVs will lead to their movement being restricted to designated aerial routes, known as \textit{UAV corridors}, which are established by relevant authorities \cite{cherif20213d, bhuyan2021secure}. As the majority of UAVs will be navigating through designated corridors, the objective for the network operators will shift from offering wide network services across the entire sky to ensuring reliable connectivity within just these corridors, as illustrated in Fig.~\ref{fig:illustration}. As the idea of UAV corridors gains popularity, researchers have been focusing on optimizing UAV trajectories, aligning the flight paths of UAVs with the optimal network coverage areas \cite{challita2018deep, bulut2018trajectory, esrafilian20203d, bayerlein2021multi}.

Nonetheless, the establishment of UAV corridors is expected to be driven by network independence and safety considerations, offering minimal flexibility for UAV trajectory adjustments and highlighting the essential demand for 3D network optimization. Recent studies have focused on adjusting cellular network deployments to cater for UAV corridors through system-level simulations or theoretical analysis of a simplified setup \cite{benzaghta2023designing, bernabe2022optimization, bernabe2023novel, maeng2023base, chowdhury2021ensuring, singh2021placement, karimi2023optimizing, karimi2023analysis}.  Despite these promising contributions, the quest for a scalable large-scale optimization framework that can effectively tackle mathematically intractable performance functions remains unmet. The proposed approaches provide foundational insights but often fall short in addressing the complex, dynamic nature of large-scale networks, as well as the lack of handling continuous or high-dimensional network configurations. The challenge lies not only in the mathematical complexity but also in ensuring the adaptability and scalability of these solutions to cater for evolving network demands, technological advancements, as well as varying users' distributions. Accordingly, there is a need for the adoption of data-driven approaches. Such approaches harness the power of existing datasets to inform and refine the optimization process; thus, greatly improving how we manage and optimize large-scale networks that can cater for users both on the ground and aerial corridors.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{
Figures/figureCorridors_v02_compressed.eps}
\caption{A cellular network featuring both downtilted and uptilted BSs, supporting ground GUEs and UAVs flying along corridors (blurred green) \cite{benzaghta2023designing}. \hl{we overused this figure, we should consider merging with Fig. 2.}}
\label{fig:illustration}
\vspace{-0.5cm}
\end{figure}

\subsection{Contribution and Summary of Results}

In this paper, we propose a new methodology based on Bayesian Optimization (BO) \cite{shahriari2015taking} to design a cellular deployment for both ground users (GUE) and UAVs flying along corridors. For traditional ground-focused networks, BO has proven useful in achieving coverage/capacity tradeoffs \cite{dreifuerst2021optimizing }, optimal radio resource allocation \cite{eller2024differentiable, zhang2023bayesian, maggi2021bayesian, tambovskiy2022cell, maggi2023energy, tekgul2021sample, tekgul2022uplink}, and mobility management \cite{de2023towards}.
A limitation of employing BO is its restraint to the optimization problem dimensions, being most effective for optimizations in continuous domains with roughly twenty or fewer decision variables\cite{frazier2018tutorial}. Consequently, this constraint on dimensionality limits the size of the cellular network that can be optimized. To mitigate this limitation, the authors in  \cite{tekgul2023joint} introduced a framework that leverages the idea of establishing a local neighborhood for each user, encompassing cells with a strong measured reference signal received power (RSRP). This approach was shown to have a linear time complexity, in contrast to the conventional cubic complexity found in BO, achieved by combining BO with differential evolution algorithms. However, the scalability of this framework depends on the neighborhood approach, as the input vector of each user is a Gaussian Process (GP) model that consists of only the parameters of its neighboring cells, which is kept the same throughout the entire optimization. Such centralized optimization methods restrict the full capabilities of BO, as learning transfer and multi-objective optimization are not feasible when the GP prior is localized. Therefore, it's essential to apply high-dimensional BO (HD-BO) techniques capable of optimizing large-scale cellular networks where the number of optimization variables surpasses 20. In HD-BO, the GP prior established at the start of the optimization contains all relevant network information, thereby enabling learning transfer and multi-objective optimization.

In this paper, we take the first step towards employing HD-BO for optimizing large-scale cellular networks that cater for both legacy GUEs and UAVs flying along corridors. First, we show the shortcoming of using vanilla-BO to optimize large-scale networks, in which the antenna parameters under optimization surpass 20. We tackle the dimensionalty issue by proposing an iterative-BO framework, as well as utilizing state-of-the-art HD-BO frameworks such as sparse axis-aligned subspaces (SAASBO) \cite{eriksson2021high}, high-dimensional Bayesian optimization via variable selection (VSBO) \cite{shen2021computationally}, and trust region BO (TuRBO) \cite{eriksson2019scalable}. We demonstrate the effectiveness and the deficiencies of each framework from a cellular network design prospective. Second, aligning with the recent vision of 3GPP Release-18 \cite{3GPP38.843} on the need for data-driven ML model generalization aiming at the development of one framework being generalizable to different scenarios and configurations, we present the generalization capability of the HD-BO framework across different scenarios (i.e., user distributions) and configurations (i.e., antenna parameters) in the content of transfer learning. Transfer learning leverages measurement outcomes from a previously performed optimization process, denoted as ‘Scenario source’ to predict the best solution for a new optimization, termed ‘Scenario target’ at the present moment. Thirdly, as many real world network applications require optimizing multiple competing black-box objectives, we demonstrate the applicability of multi-objective high-dimensional BO (MORBO), on defining a pareto front of optimal values trading off the performance of the competing objectives.

Our main findings can be summarized as follows:
\begin{itemize}[leftmargin=*]
    \item Through the optimal combinations of antenna parameters, i.e., tilts and vertical half power beamwidths (vHPBWs), which are non-obvious and difficult to design heuristically, our proposed frameworks significantly enhance coverage and users’ rates along the UAV corridors. These improvements are achieved with only a marginal reduction in ground performance compared to a baseline scenario devoid of UAVs.

    \item When evaluating uniform UAV deployment scenarios against corridor deployments, corridor deployment demonstrates improved performance, as the network requires fewer cells to cover aerial regions, resulting in an approximate 30\% increase in mean rate.
    
    \item The frameworks used draws inspiration from BO approaches to probabilistically constructing models that quickly search and narrow down the space of candidate solutions. It stands out for being both sample- and time-efficient. Remarkably, all frameworks converges within fewer than 300 iterations across all tested scenarios. This rapid convergence with minimal iterations is vital in practical deployments, as it prevents mobile operators from experimenting with parameters that might result in decreased performance.

    \item HD-BO enhances the optimization process by enabling the transfer of learning across different scenarios. This means that if an optimization scenario changes, yet bears similarity to a previous one, HD-BO can utilize existing samples without the need for additional sampling in the new scenario, conserving resources and maintaining performance levels without significant degradation. However, this efficient learning transfer is contingent upon the BO's comprehension of the environmental characteristics from the original dataset. Our experiments show that when BO is informed about UAV presence, it can adapt its knowledge from one user deployment scenario to another, i.e., changes on the characteristics of the corridors. Conversely, if BO lacks prior exposure to UAVs, learning transfer proves ineffective, particularly in scenarios where initial datasets do not include any UAV data. This limitation can lead to BO's inability to identify optimal regions for antenna adjustments, potentially resulting in suboptimal performance outcomes.

    \item \red{Summary of MORBO to be added.} 
    
\end{itemize}



\subsection{Notation and Organization}

$\cdots$

\end{comment}

%\subsection{Sum-log-rate Maximization Problem}

% Gio: Interesting paragraph but perhaps not necessary
%The focus of this work is on cell shaping, a process that tweaks antenna parameters to tailor the coverage area shape and direct main beams to targeted areas while reducing interference with adjacent cells. Cell shaping aim is to refine a cell's coverage to align with the user distribution, enhancing network coverage and capacity. It's important to highlight that cell shaping represents a long-term, cell-centric optimization strategy, predicated on the assumption of a stable user distribution. This contrasts with user-centric optimization, which adjusts more frequently to traffic fluctuations and user movements. Therefore, our study does not delve into user-specific adjustments or scenarios involving high users’ mobility.

%Furthermore, in our prior research \cite{benzaghta2023designing}, it was observed that optimizing for sum-log-SINR fails to consider the cell size, a factor that greatly influences the rate performance of the GUEs. Conversely, optimizing for sum-log-rate accounts for SINR performance, as it is a crucial element of the rate equation defined in (\ref{rates}).
%This characteristic de-emphasizes the allocation of extra resources to users who already enjoy good service, as their marginal gain in throughput minimally affects overall objective value. Conversely, enhancing the service for users with lower rates is more beneficial, as improvements here significantly boost the objective indicator.

%
%The vanilla high-dim BO is able to have an incremental enhancement on the best observed KPI; however, after 110 iterations it gets trapped in a local optima. Although the vanilla high-dim BO framework is able to deal with higher dimensions, as compared to the conventional vanilla-BO, the search space here plays a crucial part.
%

\begin{comment}
Fig.~\ref{fig:UAV_Uni_Cells} shows the resulting cell partitioning for the UAVs for the case of uniform deployment when the network is optimized for both populations of UEs, $\lambda = 0.5$. The resulting GUEs cell partitioning is shown in Fig.~\ref{fig:GUE_Uni_Cells}. Similarly, Fig.~\ref{fig:UAV_Corr_Cells} shows the resulting cell partitioning for the UAVs for the case of corridor deployment and the resulting GUEs cell partitioning is shown in Fig.~\ref{fig:GUE_Corr_Cells}.


{\begin{figure*}[!t]
    \centering
    \subfloat[Sky at 150\,m, uniform UAVs.]{
        \includegraphics[width=0.51\figwidth]{Figures/Corr_vs_Uni/2024_04_30_IterativeBO_Uni_UAV_Cells.eps}
        \label{fig:UAV_Uni_Cells}
    }
    \hspace{0.5mm}
    \subfloat[Ground at 1.5\,m, uniform UAVs.]{
        \includegraphics[width=0.51\figwidth]{Figures/Corr_vs_Uni/2024_04_30_IterativeBO_Uni_GUEs_Cells.eps}
        \label{fig:GUE_Uni_Cells}
    }
    \hspace{0.5mm}
    \subfloat[Sky at 150\,m, UAV corridors.]{
        \includegraphics[width=0.51\figwidth]{Figures/Corr_vs_Uni/2024_04_30_IterativeBO_Corr_UAV_Cells.eps}
        \label{fig:UAV_Corr_Cells}
    }
    \hspace{0.5mm}
    \subfloat[Ground at 1.5\,m, UAV corridors.]{
        \includegraphics[width=0.51\figwidth]{Figures/Corr_vs_Uni/2024_04_30_IterativeBO_Corr_GUEs_Cells.eps}
        \label{fig:corrmat_comp_a}
    }
    \caption{Cell partitioning in the sky and on the ground when the cellular network is optimized for both GUEs and UAVs ($\lambda$ = 0.5). Figures (a) and (b) refer to the case of uniformly distributed UAVs, whereas Figures (c) and (d) to the case of UAVs on corridors. \hl{Gio: Remove (a)-(b)??}}
    \label{fig:GUE_Corr_Cells}
\end{figure*}}
\end{comment}

\begin{comment}

Fig.~\ref{fig:IterativeBO_Conv_UniVSCorr} shows the convergence of the proposed iterative-BO algorithm for both UAV deployment scenarios, uniform and corridors. The iterative-BO is able to optimize both types of deployments. 

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2024_02_05_Corr_vs_Uni_bestObserved.eps}
\caption{\red{Convergence of the iterative-BO algorithm, showing the evolution of the best observed objective vs. the number of iterations $n$. (Uniform vs. Corridors)}}
\label{fig:IterativeBO_Conv_UniVSCorr}
\end{figure}

\end{comment}


\begin{comment}
\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_Uni_UAV_Cells.eps}
\caption{Sky cell partitioning (UAVs uniformly deployed) when the cellular network is optimized for both GUEs and UAVs ($\lambda$ = 0.5).}
\label{fig:UAV_Uni_Cells}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_Uni_GUEs_Cells.eps}
\caption{Ground cell partitioning (UAVs uniformly deployed) when the cellular network is optimized for both GUEs and UAVs ($\lambda$ = 0.5).}
\label{fig:GUE_Uni_Cells}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_Corr_UAV_Cells.eps}
\caption{Cell partitioning for UAV corridors when the cellular network is optimized for both GUEs and UAVs ($\lambda$ = 0.5).}
\label{fig:UAV_Corr_Cells}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_Corr_GUEs_Cells.eps}
\caption{Ground cell partitioning (UAVs in corridors) when the cellular network is optimized for both GUEs and UAVs ($\lambda$ = 0.5).}
\label{fig:GUE_Corr_Cells}
\end{figure}

\subsubsection*{Resulting performance}
Fig.~\ref{fig:SINR_CDFs_UniVSCorr} shows the cumulative distribution function (CDF) of the SINR perceived by GUEs (solid lines) and UAVs (dashed lines) when the cellular network is optimized for both users categories ($\lambda = 0.5$). The performance of a traditional cellular network (black) is also shown as a baseline for comparison, where all BSs are down-tilted to $-12^{\circ}$ as per 3GPP recommendations \cite{3GPP38901}. 
The figure shows that for the 3GPP baseline configuration, all UAVs experience SINRs below -5\,dB and thus be regarded as being in outage.%
%
\footnote{While our performance function is based on the achievable Shannon rates (\ref{rates}), practical systems employ adaptive modulation and coding schemes and require a minimum SINR to deliver a non-zero rate, typically around -5\,dB \cite{geraci2018understanding}.}
%
This behavior is expected and due to a large number of line-of-sight interfering signals of comparable strength to the signal from the serving cell \cite{GerGarAza2022}. Vertical antenna tilt optimization through the proposed iterative-BO approach significantly improves the UAV SINR, with median gains of around 13\,dB and 17\,dB for the cases of uniformly distributed UAVs (dashed red) and UAVs on corridors (dashed blue), respectively. Importantly, this SINR boost also allows to reduce the percentage of UAVs outage from 100\% to 1\% in the case of uniformly distributed UAVs and to zero in the case of corridors.
Furthermore, the UAV performance improvement does not correspond to a severe GUE performance degradation, with the GUE SINR only reduced by less than 1\,dB in median (solid black vs. solid blue/red). 


\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_UniVsCorr_SINR_CDFs.eps}
\caption{SINR for UAVs (dashed) and GUEs
(solid) when the network is optimized for both ($\lambda$ = 0.5), and for an all-downtilt baseline (3GPP).}
\label{fig:SINR_CDFs_UniVSCorr}
\end{figure}

\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\begin{comment}

%Fig.~\ref{fig:Rate_CDFs_UniVSCorr} \hl{shows the cumulative distribution function (CDF)} of the rates perceived by GUEs (solid lines) and UAVs (dashed lines) when the cellular network is optimized for both users categories ($\lambda = 0.5$). The performance of a traditional cellular network (black) is also shown as a baseline for comparison, where all BSs are down-tilted to $-12^{\circ}$ as per 3GPP recommendations \cite{3GPP38901}. The figure demonstrates that the proposed framework, in the case of corridor deployment, can optimize the cellular network in a way that boosts the UAVs rates, with a 1.52 Mbps gain in mean compared to the all-downtilt baseline (dashed blue vs. dashed black), while preserving the performance of the GUEs (solid blue vs. solid black). Similar gains can be seen in the case of uniform deployment as well, with an increase of 1.18 Mbps for the UAVs, while maintaining the same performance at the ground. 


\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_UniVsCorr_Rate_CDFs.eps}
\caption{Rate for UAVs (dashed) and GUEs (solid) when the network is optimized for both ($\lambda$ = 0.5), and for an all-downtilt baseline (3GPP).}
\label{fig:Rate_CDFs_UniVSCorr}
\end{figure}

\end{comment}

%
%The authors in \cite{eriksson2021high} proposed a function prior based on sparse axis-aligned subspaces, which assumes a hierarchy of feature relevance and encompasses a flexible class of smooth non-linear functions, allowing tractable (approximate) inference. The sparse structure  Gaussian process (GP) model in the (inverse squared) length scales $\rho_i$ is defined as
%

%
%where $\mathcal{LN}$ denotes the log-Normal distribution, $\mathcal{HC}$ denotes the half-Cauchy distribution, and $\alpha > 0$ is a hyperparameter that controls the level of shrinkage. In the SAAS function prior, the level of global shrinkage (i.e. sparsity) is controlled by the scalar $\tau > 0$, which tends to concentrate near zero due to the half-Cauchy prior. The inverse squared length scales $\rho_i$ are also subject to half-Cauchy priors, leading them to similarly concentrate close to zero. Thus, most of the dimensions are disabled "turned-off"; however, if there is sufficient evidence in the observations, the posterior over  $\tau$ will be pushed to higher values, therefore reducing the level of shrinkage and allowing more of the $\rho_i$ to escape zero, effectively ‘turning-on’ more dimensions. As data accumulates, an increasing number of the $\rho_i$ will move away from zero, leading the posterior to support a more relevant set of dimensions. This contrasts with a traditional GP fit using maximum likelihood estimation, which often leads to significant overfitting in scenarios with many dimensions.

%Given the black-box function $f(\textbf{x}) \colon \mathcal{X} \to \mathbb{R}$ in the domain $\mathcal{X} = [0,1]^D$, having a large $D$, the VSBO framework proposed in \cite{shen2021computationally} is based on the assumption that all variables in $\textbf{x}$ can be divided into important variables $\textbf{x}_{ipt}$ and unimportant variables $\textbf{x}_{nipt}$. For every $N_{vs}$ iterations, VSBO will update $\textbf{x}_{ipt}$ and $\textbf{x}_{nipt}$, and for every BO iteration only variables in $\textbf{x}_{ipt}$ are used to fit the GP model. After which, a new query of important variables is obtained by maximising the acquisition function. VSBO learns a conditional distribution $p(\textbf{x}_{nipt} \mid \textbf{x}_{ipt}, \mathcal{D})$ from the existing initial dataset $\mathcal{D}$. From this distribution the values of $\textbf{x}_{nipt}$ are chosen, such that the $f(\textbf{x})$ is maximized when $\textbf{x}_{ipt}$ is fixed. The variable selection in VSBO is performed by calculating the importance score (IS) of each variable, following a gradient-based IS calculation method, called Grad-IS. If the partial derivative of the objective function $f$ with respect to a single variable is large on average, then the variable ought to be important. However, as the derivative of $f$ is unknown, VSBO instead estimates the expectation of the gradient of posterior mean from a fitted GP model, normalized by the posterior standard deviation. VSBO sequentially selects variables based on their IS, and upon adding a new variable, the algorithm refits the GP using only the selected variables, subsequently recording a new final loss. If the new loss closely matches the previous loss, which is the loss of the fitted GP when the new variable is excluded, then the selection process terminates, and all selected variables up to that point are deemed important. VSBO automatically learn axis-aligned sub-spaces, i.e. spaces containing selected variables, without the demand of any pre-specified hyperparameters.

%Therefore, $\tau_{succ}, \tau_{fail}, L_{init}, L_{min}, \text{and} L_{max}$ are the hyperparameters of the TuRBO framework.

\begin{comment}
To address the high dimensionality issue of BO, the authors in \cite{eriksson2019scalable} proposed to move away from global surrogate modeling and instead aim for global optimization by managing multiple independent local models, each involved in a separate local optimization run. In TuRBO, to reach global optimization, the framework simultaneously manage several local models and allocate samples using an implicit multi-armed bandit strategy. This approach results in an effective acquisition strategy that guides samples towards promising local optimization runs. To achieve local optimization in a gradient-free setting, TuRBO draw inspiration from a class of trust region (TR) methods from stochastic optimization. Such techniques propose recommendations by employing a simple surrogate model within a TR, which is typically shaped as a sphere or a polytope centered around the best solution. Within this region, the surrogate model is considered to accurately represent the function.  However, simple surrogate models might require overly small trust regions to provide accurate modeling behavior; thus, TuRBO usesm a GP surrogate model within a TR. This enables the framework to adopt the global BO robustness to noise, as well as its rigorous reasoning about uncertainty. In TuRBO, the TR is chosen to be a hyperrectangle centered at the best solution found so far $f^{*}$. At the start of a given local optimization run, the base side length of the TR is initialized to $ L \gets L_{init}$. Then, the actual side length for each dimension is determined by rescaling this base side length in accordance with its lengthscale $\lambda_{i}$ in the GP model, while preserving a total volume of $L^{d}$. Thus, the  actual side length is defined as
\begin{equation}
L_i = \lambda_i L / \left( \prod_{j=1}^{d} \lambda_j \right)^{1/d}
\end{equation}
To carry out a single local optimization run, an acquisition function is used at each iteration to select a batch of q candidates, ensuring they are confined within the TR. If the size of $L$ were large enough for the TR to encompass the entire space, this approach would essentially be equivalent to running standard global BO. Consequently, the adjustment of $L$ plays a crucial role. On one hand, the TR needs to be large enough to encompass good solutions. On the other hand, it should remain compact to guarantee the local model's accuracy within the TR. The common practice involves expanding the TR when the optimizer makes progress, i.e., it finds better solutions in that region,and shrink it when the optimizer appears stuck. Thus, after $\tau_{succ}$ consecutive successes, the framework  double the size of the TR, i.e., $L \gets \min \{L_{max}, 2L\}$, whereas after $\tau_{fail}$ consecutive failures, the size of the TR is halved $L \gets L/2$. The success and failure counters are reset to zero after the change in the TR. Whenever $L$ drops below a specified minimum threshold, $L_{min}$, the corresponding TR is discarded, and a new one is initiated with a side length of $L_{init}$. Moreover, the side length can not exceed a maximum threshold, $L_{max}$. Therefore, $\tau_{succ}, \tau_{fail}, L_{init}, L_{min}, \text{and} L_{max}$ are the hyperparameters of the TuRBO framework.  TuRBO maintains $m$ trust regions simultaneously, in which each trust region $\text{TR}_{l}$ with $l \in \{1, \dots, m\}$ is a hyperrectangle of base side length $L_{l} \leq L_{max}$, and utilizes an independent local GP model. This creates a classic exploitation-exploration dilemma, which TuRBO address using a multi-armed bandit approach that considers each TR as a separate lever. 
At every iteration,  the framework choose a batch of q candidates drawn from the union of all trust regions and then update all local optimization tasks from which these candidates were selected. Thompson sampling is used for selecting candidates within a single TR, as well as selecting candidates across the set of trust regions simultaneously.
\end{comment}

%By doubling the optimization paramters (i.e., from 57 tilts to 57 tilts + 57v-HPBW), TuRBO is demonstrated to have linear time complexity as opposed to cubic in vanilla-BO, making it a sample- and time-efficient  algorithm suited for such large-scale network optimizations.

\begin{comment}

Fig.~\ref{fig:Opt_HDBO_EK_compare_bar} shows a comparison of the achieved rates in terms of 10\%-tile, 50\%-tile, 90\%-tile  of both GUEs and UAVs, for vanilla-BO, iterative-BO, and TuRBO. As expected, it is observed that vanilla-BO performance the worse, for both type of users. TuRBO perform similar to the iterative-BO for the GUEs, whereas it achieves better performance for the UAVs. 

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Iterative_vs_HighDim/2023_12_15_Iterative_vs_TuRBO_barGraph.eps}
\caption{Achieved rates comparison (10\%-tile, 50\%-tile, 90\%-tile) of both GUEs and UAVs.}
\label{fig:Opt_HDBO_EK_compare_bar}
\end{figure}

\end{comment}

\begin{comment}
Fig.~\ref{fig:Tilts_vHPBW_conv_TuRBO} shows the convergence performance of TuRBO by illustrating the best observed KPI objective at each iteration $n$. By doubling the optimization paramters (i.e., from 57 tilts to 57 tilts + 57v-HPBW), the algorithm is demonstrated to have linear time complexity as opposed to cubic in vanilla-BO, making it a sample- and time-efficient  algorithm suited for such large-scale network optimizations.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/tilts_and_vHPBW/2024_02_06_TuRBO_TiltandVHPBW_bestObserved.eps}
\caption{Convergence of the algorithms, showing the evolution of the best observed objective vs. the number of iterations $n$.}
\label{fig:Tilts_vHPBW_conv_TuRBO}
\end{figure}

\end{comment}

\begin{comment}
\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/tilts_and_vHPBW/2023_12_30_Corr_TiltandVHPBW_TuRBO_SINR_CDFs.eps}
\caption{SINR for UAVs (dashed) and GUEs
(solid) when the network is optimized for both ($\lambda$ = 0.5), and for an all-downtilt, full-power baseline (3GPP).}
\label{fig:SINR_CDFs_tilts_vHPBW}
\end{figure}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

Fig.~\ref{fig:Rate_CDFs_tilts_vHPBW} shows the CDF of the rates perceived by the GUEs and the UAVs.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/tilts_and_vHPBW/2023_12_30_Corr_TiltandVHPBW_TuRBO_Rate_CDFs.eps}
\caption{Rates for UAVs (dashed) and GUEs
(solid) when the network is optimized for both ($\lambda$ = 0.5), and for an all-downtilt, full-power baseline (3GPP).}
\label{fig:Rate_CDFs_tilts_vHPBW}
\end{figure}

\end{comment}

\begin{comment}

    \begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_Corr_50m_150m/2024_02_06_LT_Corr_Hight_50m_150m_bestObserved.eps}
\caption{Convergence of the scenario-based learning tranfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$. Scenario target: GUEs and UAVs along corridors at 50m. Scenario source: GUEs and UAVs along corridors at 150m.}
\label{fig:LT_conv_50m_150m}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_UAVs_noUAVs/2024_02_28_LT_Corr150m_NoUAVs_bestObserved.eps}
\caption{Convergence of the scenario-based learning tranfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$. Scenario target: GUEs and UAVs along corridors at 150m. Scenario source:  GUEs only without UAVs.}
\label{fig:LT_conv_UAVs_NoUAVs}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_Corr_30deg_10deg/2024_02_06_LT_Corr_Hight_50m_30deg_10deg_bestObserved.eps}
\caption{Convergence of the configuration-based learning transfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$. Scenario target: BSs antenna vHPBW of 10 deg. Scenario source: BSs antenna vHPBW of 30 deg.}
\label{fig:LT_conv_30deg_10deg}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_Corr_50m_150m/2023_12_20_LT_corr50m150m_barGraph.eps}
\caption{Convergence of the scenario-based learning tranfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$. Scenario target: GUEs and UAVs along corridors at 50m. Scenario source: GUEs and UAVs along corridors at 150m }
\label{fig:LT_compare_50m_150m_bar}
\end{figure}
$\cdots$

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_UAVs_noUAVs/2024_03_06_LT_Corr150m_NoUAVs_barGraphs.eps}
\caption{Convergence of the scenario-based learning tranfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$. Scenario target: GUEs and UAVs along corridors at 150m. Scenario source:  GUEs only without UAVs.}
\label{fig:LT_compare_UAVs_NoUAVs}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_Corr_30deg_10deg/2023_12_28_LT_Corr_Hight_50m_30deg_10deg_barGraph.eps}
\caption{Convergence of the configuration-based learning tranfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$. Scenario target: BSs antenna vHPBW of 10 deg. Scenario source: BSs antenna vHPBW of 30 deg.}
\label{fig:LT_compare_30deg_10deg_bar}
\end{figure}

\end{comment}

\begin{comment}
Simultaneous optimization of capacity and coverage is a key issue in the deployment and configuration of wireless cellular networks. Given the intricate nature of network setup and the abundance of performance-related data, data-driven approaches are particularly well-suited to address this challenge \cite{lin2023overview}. As data collection capabilities of cellular networks increase, there are more opportunities to tackle capacity-coverage tradeoff with ML approaches, specifically BO techniques \cite{dreifuerst2021optimizing}.

Ensuring reliable coverage for UAVs involves directing energy upwards by up-tilting the sectors, which leads to reduced performance rates for the GUEs who benefit from sectors being down-tilted. In this section, we propose optimizing both the UAVs' coverage and the GUEs' capacity in a multi-cell network through the adjustment of each sector's vertical antenna tilt. We approach the capacity and coverage objectives as black-box functions, which lack explicit analytical expressions and gradient observations. Our objective is to maximize coverage and capacity by strategically optimizing the vertical tilt angles of each sector within a defined range $\chi \subset \mathbb{R}^d$. In this multi-objective optimization problem, there isn't one definitive best solution; instead, the aim is to determine a set of Pareto optimal solutions. In these solutions, any enhancement in UAVs' coverage will result in a reduction in GUEs' capacity, and vice versa.
\end{comment}

\begin{comment}
{\begin{figure*}[!t]
    \centering
    \subfloat[Uniformly distributed UAVs]{
        \includegraphics[width=0.98\columnwidth]{Figures/Multi_Obj/2024_04_26_MORBO_300m_PcUAVs_RateGUEs_ninesReliability_Pareto_Uni.eps}
        \label{fig:MORBO_PcUAVs_RatesGUEs_uniform}
    }
    \hspace{1mm}
    \subfloat[UAVs on corridors]{
        \includegraphics[width=0.98\columnwidth]{Figures/Multi_Obj/2024_04_26_MORBO_300m_PcUAVs_RateGUEs_ninesReliability_Pareto.eps}
        \label{fig:MORBO_PcUAVs_RatesGUEs_corridors}
    }
    \caption{Complete search space with all samples obtained through the MORBO framework: (a) UAVs uniformly distributed, (b) UAVs on corridors. The color bar indicates the iteration number, while the solid black line depicts the Pareto front obtained. \hl{Md: Shall we only keep (b) and copy paste the Pareto front from (a) in (b) in black dashed line?}}
    \label{fig:MORBO_PcUAVs_RatesGUEs}
    \hspace{2mm}
\end{figure*}}
\end{comment}

\begin{comment}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Multi_Obj/2024_03_24_MORBO_300m_PcUAVs_RateGUEs_ninesReliability_Pareto.eps}
\caption{Complete search space with all samples obtained through the MORBO framework. Pareto-front obtained is indicated with the solid black line (Corridor deployment).}
\label{fig:MORBO_PcUAVs_RatesGUEs}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Multi_Obj/2024_04_08_MORBO_300m_PcUAVs_RateGUEs_ninesReliability_Pareto_Uni.eps}
\caption{Complete search space with all samples obtained through the MORBO framework. Pareto-front obtained is indicated with the solid black line (Uniform deployment).}
\label{fig:MORBO_PcUAVs_RatesGUEs}
\end{figure}

\end{comment}


\begin{comment}

Fig.~\ref{fig:SINR_CDFs_RD} shows the cumulative distribution function (CDF) of the SINR perceived by GUEs (solid lines) and UAVs (dashed lines) when the cellular network is optimized for both GUEs and UAV corridors ($\lambda = 0.5$), by jointly tuning antenna tilts and HPBW. 
%
The performance achieved by the cellular network with its original configuration of cell tilts and HPBW (black) is also shown as a baseline for comparison. The figure shows that under the baseline configuration, 45\% of the UAVs would experience SINRs below -5\,dB and could thus be regarded as being in outage (dashed black). The joint optimization of vertical antenna tilts and HPBW through TuRBO HD-BO improves the SINR along UAV corridors, reducing the percentage of UAVs in outage from 45\% to 4\%. Remarkably, this UAV performance improvement does not correspond to a severe GUE performance degradation (solid black vs. solid blue). 

\begin{figure}
\centering
\includegraphics[width=0.99\columnwidth]{Figures/Real_Deployment/2024_05_03_RD_SINR_GUEs_UAVs_Corr_TuRBO.eps}
\caption{SINR for UAVs (dashed) and GUEs
(solid) when the network is optimized for both ($\lambda$ = 0.5), and for an all-downtilt real-deployment configuration.}
\label{fig:SINR_CDFs_RD}
\end{figure}

\end{comment}

%%% MOVED TO THE CONCLUSIONS %%%
\begin{comment}
While we refer the reader to the body of the article for a comprehensive collection of results and discussions, the following list serves as a preview of the most important takeaways from our study:

\begin{itemize}%[leftmargin=*]

\item 
\emph{Optimal design for UAV corridors:}
An optimal combination of vertical antenna tilts and vertical half-power beamwidth (HPBW), which are non-obvious and challenging to design heuristically, allows to significantly enhance the performance along the UAV corridors. An optimized setup yields gains exceeding 20\,dB in median SINR with respect to an all-downtilt, fixed-HPBW 3GPP baseline. These improvements are achieved with only a marginal reduction in ground performance compared to a scenario devoid of UAVs. When compared to uniformly distributed UAVs, the network requires fewer cells to cover UAVs along corridors, \red{resulting in a 30\% increase in mean rate.} \hl{Md check, which case?}

\item
\emph{Efficiency and convergence of HD-BO:}
HD-BO draws inspiration from BO to construct data-driven models that efficiently search and narrow down the space of candidate solutions. While exhibiting different final performance---with TuRBO showing remarkable superiority---, all HD-BO approaches considered converge within fewer than 300 iterations across all tested scenarios. This rapid convergence is crucial in practical deployments, preventing network designers from experimenting with parameters that might lead to decreased performance.

\item
\emph{Successful vs. unsuccessful transfer learning:}
HD-BO enhances the optimization process by enabling transfer learning across different scenarios. This means if an optimization scenario changes but is similar to a previous one, HD-BO can utilize existing samples without needing additional sampling in the new scenario, conserving resources and maintaining performance levels without significant degradation. However, this efficient learning transfer depends on the BO’s understanding of the environmental characteristics from the original dataset. Our experiments demonstrate that when BO is informed about UAV presence, it can adapt its knowledge from one user deployment scenario to another, adjusting to changes in the characteristics of the corridors. Conversely, if BO lacks prior exposure to UAVs, learning transfer proves ineffective, particularly in scenarios where initial datasets do not include any UAV data. This limitation can lead to BO’s inability to identify optimal regions for antenna adjustments, potentially resulting in suboptimal performance outcomes.

\item
\emph{Coverage-capacity trade-offs:}
Multi-objective HD-BO allows to effectively trade-off GUE data rates for UAV coverage reliability, with UAV corridors allowing to achieve superior trade-offs. For instance, when UAVs are uniformly distributed---and thus UAV coverage is pursued across the entire sky---, achieving three `nines' of reliability incurs GUE rates one third lower than in the case of UAV corridors. Likewise, for a given GUE geometrical mean rate of 1.3\,Mbps, nearly four `nines' or reliability can be guaranteed with UAV corridors as opposed to three `nines' with uniform UAVs.

\item
\emph{Performance in a site-specific scenario:}
Our case study of a production cellular network confirms the results obtained under 3GPP statistical models, with HD-BO identifying optimal antenna tilts and HPBW configurations that more than double the UAV rates while incurring a negligible performance reduction for GUEs.

\end{itemize}
\end{comment}

\begin{comment}
\begin{equation}
A_{\text{H}}(\phi)_{\textrm{dB}} = - \min \left[ 12 \left( \frac{\phi - \phi^{b}}{\phi_{\text{3dB}}} \right)^2, 25 \right] \, ,
\end{equation}
\begin{equation}
A_{\text{V}}(\theta)_{\textrm{dB}} = - \min \left[ 12 \left( \frac{\theta - \theta^{b}}{\theta_{\text{3dB}}} \right)^2, 25 \right] \, .
\end{equation}
\end{comment}

\begin{comment}
\begin{figure}
\centering
\includegraphics[width=\figwidth]{
Figures/figureCorridors_v02_compressed.eps}
\caption{A cellular network featuring both downtilted and uptilted BSs, supporting ground GUEs and UAVs flying along corridors (blurred green) \cite{benzaghta2023designing}. \hl{Merge this with Fig. 2.}}
\label{fig:illustration}
\vspace{-0.5cm}
\end{figure}
\end{comment}

\begin{comment}
\begin{algorithm}[hbt!]
\caption{Proposed iterative-BO algorithm}\label{alg:BO}
\textbf{Input:} Initial dataset $\mathcal{D} = \{\textbf{x}_1,\ldots,\textbf{x}_{N_{\textrm{o}}},\tilde{f}_1,\ldots,\tilde{f}_{N_{\textrm{o}}}\}$;

\textbf{Output:} Optimal configuration $\textbf{x}^{*}$;

\textbf{Initialization:}

\quad Create a GP prior $\{\mu(\cdot), k(\cdot, \cdot)\}$ using $\mathcal{D}$ and (\ref{posterior});

\quad Set all entries of $\bm{\theta}_0$ to $0^{\circ}$;

%\quad Set all entries of $\bm{p}_0$ to $46~\text{dBm}$;

\quad Set $\textbf{x}_0 = \bm{\theta}_0$, $n = \ell=1$, $\ell_{\textrm{max}} = 3$, $\tilde{f}^{*} = \tilde{f}_0^{*} = -\infty$;

%\quad Set $n = 1$, $\ell=1$, $\ell_{\textrm{max}} = 3$, $\tilde{f}^{*} = \tilde{f}_0^{*} = -\infty$;

\While{$\ell \leq \ell_{\emph{max}}$}{
$b_{n} = ((n-1) \mod \|\ncalB\|) + 1$; 

Draw $N_{\textrm{c}}$ random candidate points $\{\widehat{x}_{\text{cand}_{1}},\ldots,\widehat{x}_{\text{cand}_{N_{\textrm{c}}}}\}$;

Evaluate all candidate points using \eqref{eqn:EI};

Obtain $\widehat{x}_{n} = \theta_{b_{n}}$ from \eqref{eqn:BO_acq};

Update $\textbf{x}_{n}$ with $\theta_{b_{n}}$;

Obtain observation $\tilde{f}_n = \tilde{f}(\textbf{x}_n)$ using \eqref{eqn:Opt_problem};

Augment $\mathcal{D}$ by including $\textbf{x}_{n}$ and $\tilde{f}_n$;

Update the GP prior $\{\mu(\cdot), k(\cdot, \cdot)\}$ using $\mathcal{D}$ and (\ref{posterior});

\If{$\tilde{f}_{n} > \tilde{f}^{*}_{n-1}$}
{$\tilde{f}_n^{*} \gets\tilde{f}_{n}$;
$\textbf{x}_{n}^{*} \gets \textbf{x}_{n}$;
}
\Else{$\tilde{f}_n^{*} \gets \tilde{f}^{*}_{n-1}$;
}

\If{$b_n=\|\ncalB\|$}
{
\If{$\tilde{f}^{*}_{n} > \tilde{f}^{*}$}
{$\tilde{f}^{*} \gets \tilde{f}^{*}_{n}$;
$\textbf{x}^{*} \gets \textbf{x}_{n}^{*}$;
$\ell \gets 0$;
}
{$\ell \gets \ell + 1$;
}}
$n \gets n + 1$;
}
\end{algorithm}
\end{comment}

\begin{comment}
Since the objective function defined in (\ref{eqn:Opt_problem}) has a logarithmic value, which does not represent any meaningful insight from a wireless communication prospective, throughout this paper, we demonstrate the best observed objective value $f^{*}$ as the geometrical mean of the users' rate, which is defined as $ \overline{\mathcal{R}} = \left( \prod_{n=1}^{k} x_n \right)^{\frac{1}{k}}$. Note that the geometric mean $\overline{\mathcal{R}}$ can be mapped to the objective $f(.)$ in (\ref{eqn:Opt_problem}), for the case of $\lambda=0.5$, as $\overline{R} = \exp\left(\frac{f}{k}\right)$.

Random search is also shown as a baseline, in which the tilts are uniformly sampled from the search space $[-20^{\circ}, 45^{\circ}]$. As can be seen from the graph, the vanilla BO approach is not able to optimize high dimensional problems (i.e., 57-dimensions in this scenario, resulting from 57 cells, in which each cell needs to optimize its corresponding antenna tilt). Optimizing for both down-tilts and up-tilts results in a wide search space ranging in  $[-20^{\circ}, 45^{\circ}]$, which results in a sub-optimal local solution. The proposed iterative-BO framework tackles both of those drawback that the vanilla-BO approaches had, resulting in a better convergence performance and avoiding sub-optimal local solutions. In the iterative-BO approach, convergence is reached in 130 iterations, with a KPI value increase of 175\%.
\end{comment}

\begin{comment}

\subsubsection*{Takeaways}

In this section, we demonstrated that optimizing the vertical antenna tilts in a cellular network can be an effective approach to support connectivity along UAV corridors without jeopardizing the performance of legacy GUEs. 
We successfully carried out such optimization by proposing iterative-BO and thus overcoming the limitations of vanilla-BO in handling a large number of optimization variables. 
%
However, we note that the GP prior created by iterative-BO is not generalized to the whole search space, but rather a local prior specific to the BS tilt being optimized at each iteration. This shortcoming prevents applying iterative-BO to carry out transfer learning across different scenarios or tackle multi-objective optimization problems.
%
To overcome this issue, in Section~\ref{sec:HD-BO} we extend our study to identify high-dimensional Bayesian optimization methods capable of handling high-dimensional search spaces while maintaining a general prior. This then allows us to apply transfer learning in Section~\ref{sec:TL} and to carry out multi-objective optimization in Section~\ref{sec:MORBO}.

\end{comment}

==> Results.tex <==
\section{Simulations}

$\cdots$

\subsection{Iterative-BO vs. vanilla approaches}

Fig.~\ref{fig:Opt_vanilla_conv_compare} compares the convergence performance of the vanilla BO and vanilla high-dim BO to the  proposed iterative-BO algorithm by illustrating the best observed KPI objective at each iteration $n$. Random search is also shown as a baseline, in which the tilts are uniformly chosen from the search space $[ \,-20, 45] \,$ deg. As can be seen from the graph, the vanilla BO approach is not able to optimize high dimensional problems (i.e., 57-dimensions in this scenario, resulting from 57 cells, in which each cell needs to optimize its corresponding antenna tilt). The vanilla high-dim BO is able to have an incremental enhancement on the best observed KPI; however, after 110 iterations it gets trapped in a local optima. Although the high-dim BO framework is able to deal with higher dimensions, as compared to the conventional vanilla BO, the search space here plays a crucial part. Optimizing for both down-tilts and up-tilts results in a wide search space ranging in  $[ \,-20, 45] \,$) deg, which results in a sub-optimal local solution. The proposed iterative-BO framework tackles both of those drawback that the vanilla BO approaches had, resulting in a better convergence performance and avoiding sub-optimal local solutions. In the iterative-BO approach, convergence is reached in 130 iterations, with a KPI value increase of 175\%.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Iterative_vs_Vanilla/2024_02_05_IterativeBO_vs_Vanilla_bestObserved.eps}
\caption{Convergence of the algorithms, showing the evolution of the best observed objective vs. the number of iterations $n$.}
\label{fig:Opt_vanilla_conv_compare}
\end{figure}

Fig.~\ref{fig:Opt_vanilla_Rate_compare} shows a comparison of the achieved rates in terms of 10\%-tile, 50\%-tile, 90\%-tile of both GUEs and UAVs. The iterative-BO approach enhances the rates of the GUEs by a factor of 1.46, 1.36, 1.2, for the  10\%-tile, 50\%-tile, 90\%-tile, respectively.  Similarly, the UAVs rates are increased by a factor of 1.43 and 1.14, for the 50\%-tile and 90\%-tile, respectively.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Iterative_vs_Vanilla/2023_10_04_Vanilla_vs_Iterative_barGraph.eps}
\caption{Achieved rates comparison (10\%-tile, 50\%-tile, 90\%-tile) of both GUEs and UAVs}
\label{fig:Opt_vanilla_Rate_compare}
\end{figure}

$\cdots$

\subsection{Corridors vs. Uniform deployments}

Fig.~\ref{fig:IterativeBO_Conv_UniVSCorr} shows the convergence of the proposed iterative-BO algorithm by illustrating the best observed objective at each iteration $n$, for both UAV deployment scenarios, uniform and corridors. The iterative-BO is able to optimize both types of deployments. A better performance is achieved in the case of corridors deployment as the network uses fewer cells to cover the sky. The optimum configuration resulted in up-tilting 12 BSs for the case of corridors, compared to 17 up-tilted BSs for the uniform deployment scenario.

Fig.~\ref{fig:Opt_values_tilt} shows the optimal values of the vertical electrical antenna tilts $\bm{\theta}$ for the case $\lambda=0.5$, where a tradeoff is sought between rates on the ground and along the sky. The BS index denotes the deployment site (black dots in Fig.~\ref{fig:UAV_Corr_Cells}), each comprising three sectors (cells). Markers indicate whether each cell is serving GUEs (green circles) or UAVs (blue diamonds). The figures show that, unlike a traditional cellular network configuration where all BSs are downtilted (e.g., to $-12^{\circ}$ \cite{3GPP38901}), pursuing a tradeoff between the ground and the UAV corridors results in a subset of the BSs being uptilted (i.e., a total of 12 BSs in the case of corridor deployment and 17 for uniform case), with the rest remaining down-tilted. Such configuration is non-obvious and would be difficult to design heuristically.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2024_02_05_Corr_vs_Uni_bestObserved.eps}
\caption{Convergence of the iterative-BO algorithm, showing the evolution of the best observed objective vs. the number of iterations $n$. (Uniform vs. Corridors)}
\label{fig:IterativeBO_Conv_UniVSCorr}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_Corr_Uni_Config.eps}
\caption{Optimized BS tilts for both GUEs and UAVs ($\lambda = 0.5$). Green circles, blue diamonds, denote BSs serving GUEs and serving UAVs, respectively.}
\label{fig:Opt_values_tilt}
\end{figure}

Fig.~\ref{fig:UAV_Uni_Cells} shows the resulting cell partitioning for the UAVs for the case of uniform deployment when the network is optimized for both populations of UEs, $\lambda = 0.5$. The resulting GUEs cell partitioning is shown in Fig.~\ref{fig:GUE_Uni_Cells}. Similarly, Fig.~\ref{fig:UAV_Corr_Cells} shows the resulting cell partitioning for the UAVs for the case of corridor deployment and the resulting GUEs cell partitioning is shown in Fig.~\ref{fig:GUE_Corr_Cells}.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_Uni_UAV_Cells.eps}
\caption{Sky cell partitioning (UAVs uniformly deployed) when the cellular network is optimized for both GUEs and UAVs ($\lambda$ = 0.5).}
\label{fig:UAV_Uni_Cells}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_Uni_GUEs_Cells.eps}
\caption{Ground cell partitioning (UAVs uniformly deployed) when the cellular network is optimized for both GUEs and UAVs ($\lambda$ = 0.5).}
\label{fig:GUE_Uni_Cells}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_Corr_UAV_Cells.eps}
\caption{Cell partitioning for UAV corridors when the cellular network is optimized for both GUEs and UAVs ($\lambda$ = 0.5).}
\label{fig:UAV_Corr_Cells}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_Corr_GUEs_Cells.eps}
\caption{Ground cell partitioning (UAVs in corridors) when the cellular network is optimized for both GUEs and UAVs ($\lambda$ = 0.5).}
\label{fig:GUE_Corr_Cells}
\end{figure}

Fig.~\ref{fig:Rate_CDFs_UniVSCorr} shows the cumulative distribution function (CDF) of the rates perceived by GUEs (solid lines) and UAVs (dashed lines) when the cellular network is optimized for both users categories ($\lambda = 0.5$, blue). The performance of a traditional cellular network (black) is also shown as a baseline for comparison, where all BSs are down-tilted to $-12^{\circ}$ and transmit at full power as per 3GPP recommendations \cite{3GPP38901}. The figure demonstrates that the proposed framework, in the case of corridor deployment, can optimize the cellular network in a way that boosts the UAVs rates, with a 1.52 Mbps gain in mean compared to the all-downtilt, full-power baseline (dashed blue vs. dashed black), while preserving the performance of the GUEs (solid blue vs. solid black). Similar gains can be seen in the case of uniform deployment as well, with an increase of 1.18 Mbps for the UAVs, while maintaining the same performance at the ground. 
 

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_UniVsCorr_Rate_CDFs.eps}
\caption{Rate for UAVs (dashed) and GUEs (solid) when the network is optimized for both ($\lambda$ = 0.5), and for an all-downtilt, full-power baseline (3GPP).}
\label{fig:Rate_CDFs_UniVSCorr}
\end{figure}

The CDF of the SINR perceived by the GUEs and the UAVs are shown in Fig.~\ref{fig:SINR_CDFs_UniVSCorr}. The figure shows that for the 3GPP baseline configuration, all of the UAVs are in outage, due to their high altitudes and the absence of side-lobes. The proposed framework significantly boosted the SINR of the UAVs, reducing the outage to 0\% and 1\% for the deployment case of corridors and uniform, respectively. The SINR for the GUEs fell short of the baseline performance by 1\% of the GUEs being in outage.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Corr_vs_Uni/2023_10_05_IterativeBO_UniVsCorr_SINR_CDFs.eps}
\caption{SINR for UAVs (dashed) and GUEs
(solid) when the network is optimized for both ($\lambda$ = 0.5), and for an all-downtilt, full-power baseline (3GPP).}
\label{fig:SINR_CDFs_UniVSCorr}
\end{figure}

$\cdots$

\subsection{High-dim BO vs. Iterative-BO}

Fig.~\ref{fig:Opt_HDBO_EK_compare} shows the convergence of the proposed high-dim BO with expert knowledge algorithm compared to the vanilla high-dim BO approach and the iterative-BO framework, illustrating the best observed objective at each iteration $n$. 

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Iterative_vs_HighDim/2024_02_06_HighdimBO_bestObserved.eps}
\caption{Convergence of the algorithms, showing the evolution of the best observed objective vs. the number of iterations $n$.}
\label{fig:Opt_HDBO_EK_compare}
\end{figure}

Fig.~\ref{fig:Opt_HDBO_EK_compare_bar} shows a comparison of the achieved rates in terms of 10\%-tile, 50\%-tile, 90\%-tile  of both GUEs and UAVs.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/Iterative_vs_HighDim/2023_12_15_Iterative_vs_TuRBO_barGraph.eps}
\caption{Achieved rates comparison (10\%-tile, 50\%-tile, 90\%-tile) of both GUEs and UAVs}
\label{fig:Opt_HDBO_EK_compare_bar}
\end{figure}

$\cdots$
\begin{comment}
High-dim BO Expert Knowldgee (HDBO-EK): In this approach, I start the HDBO on a specific subset of the search space, from which the HDBO will understand the behaviour of the network, determining the cells that should be up-tilted or down-tilted. From there, the framework will optimize the up-tilted cells on a specific search space which suits the up-tilts better, then the HDBO-EK moves to optimizing the down-tilted cells based on a search space that enhances the performance of the down-tilts cells (hyper parameter $\alpha$ is fixed in this method to 0.1, making the framework uncorrelated to it's effect; thus, learning transfer would be possible
\end{comment}

\subsection{Learning Transfer}

Fig.~\ref{fig:LT_conv_50m_150m} shows the convergence of the scenario-based learning transfer of the proposed HDBO-EK algorithm, illustrating the best observed objective at each iteration $n$. The learning transfer is applied for a scenario change category, in which the scenario target consist of GUEs and UAVs along corridors at 50m, whereas scenario source is based on GUEs and UAVs deployed at 150m height corridors. In Fig.~\ref{fig:LT_compare_50m_150m_bar} a comparison of the achieved rates in terms of 10\%-tile, 50\%-tile, 90\%-tile  of both GUEs and UAVs are shown. 


\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_Corr_50m_150m/2024_02_06_LT_Corr_Hight_50m_150m_bestObserved.eps}
\caption{Convergence of the scenario-based learning tranfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$.}
\label{fig:LT_conv_50m_150m}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_Corr_50m_150m/2023_12_20_LT_corr50m150m_barGraph.eps}
\caption{Convergence of the scenario-based learning tranfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$.}
\label{fig:LT_compare_50m_150m_bar}
\end{figure}

Fig.~\ref{fig:LT_conv_30deg_10deg} shows the convergence of the configuration-based learning transfer of the proposed HDBO-EK algorithm, illustrating the best observed objective at each iteration $n$. The learning transfer is applied for a configuration change category, in which the scenario target consist of GUEs and UAVs along corridors at 50m with antenna vHPBW of 10 deg, whereas scenario source is based on GUEs and UAVs deployed at 50m height corridors with antenna vHPBW of 30 deg. In Fig.~\ref{fig:LT_compare_30deg_10deg_bar} a comparison of the achieved rates in terms of 10\%-tile, 50\%-tile, 90\%-tile  of both GUEs and UAVs are shown. 


\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_Corr_30deg_10deg/2024_02_06_LT_Corr_Hight_50m_30deg_10deg_bestObserved.eps}
\caption{Convergence of the configuration-based learning transfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$.}
\label{fig:LT_conv_30deg_10deg}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/LT_Corr_30deg_10deg/2023_12_28_LT_Corr_Hight_50m_30deg_10deg_barGraph.eps}
\caption{Convergence of the configuration-based learning tranfer approach, showing the evolution of the best observed objective vs. the number of iterations $n$.}
\label{fig:LT_compare_30deg_10deg_bar}
\end{figure}

$\cdots$

\subsection{Multi-variable optimization (tilts+ vertical HPBW)}

Fig.~\ref{fig:Tilts_vHPBW_conv_TuRBO} shows the convergence performance of the proposed high-dim BO framework by illustrating the best observed KPI objective at each iteration $n$. Fig.~\ref{fig:Opt_Tilts_vHPBW_config_TuRBO} shows the optimal values of the vertical electrical antenna tilts $\bm{\theta}$ and the vertical HPBW $\bm{\phi}_{3dB}$ for the case $\lambda=0.5$, where a tradeoff is sought between rates on the ground and along the sky. The BS index denotes the deployment site (black dots in Fig.~\ref{fig:UAV_Corr_Cells}), each comprising three sectors (cells). Markers indicate whether each cell is serving GUEs (green circles) or UAVs (blue diamonds).

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/tilts_and_vHPBW/2024_02_06_TuRBO_TiltandVHPBW_bestObserved.eps}
\caption{Convergence of the algorithms, showing the evolution of the best observed objective vs. the number of iterations $n$.}
\label{fig:Tilts_vHPBW_conv_TuRBO}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/tilts_and_vHPBW/2023_12_30_TuRBO_TiltandVHPBW_config.eps}
\caption{Optimized BS tilts and vHPBWs for both GUEs and UAVs ($\lambda = 0.5$). Green circles, blue diamonds, denote BSs serving GUEs and serving UAVs, respectively.}
\label{fig:Opt_Tilts_vHPBW_config_TuRBO}
\end{figure}

The CDF of the SINR perceived by the GUEs and the UAVs are shown in Fig.~\ref{fig:SINR_CDFs_tilts_vHPBW}. The figure shows that when optimizing for both tilts and vHPBW,the 50\%-tile SINR of the UAVs is increased by 4.2dB, while maintaining the same performance for the GUEs. Similar enhancement can be seen in terms of rates as well, Fig.~\ref{fig:Rate_CDFs_tilts_vHPBW} shows the CDF of the rates perceived by the GUEs and the UAVs.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/tilts_and_vHPBW/2023_12_30_Corr_TiltandVHPBW_TuRBO_SINR_CDFs.eps}
\caption{SINR for UAVs (dashed) and GUEs
(solid) when the network is optimized for both ($\lambda$ = 0.5), and for an all-downtilt, full-power baseline (3GPP).}
\label{fig:SINR_CDFs_tilts_vHPBW}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/tilts_and_vHPBW/2023_12_30_Corr_TiltandVHPBW_TuRBO_Rate_CDFs.eps}
\caption{SINR for UAVs (dashed) and GUEs
(solid) when the network is optimized for both ($\lambda$ = 0.5), and for an all-downtilt, full-power baseline (3GPP).}
\label{fig:Rate_CDFs_tilts_vHPBW}
\end{figure}

\subsection{Multi-objective}

\begin{comment}
\[
\xi = \frac{\sum_{k=1}^{K} \mathbbm{1}_{\{\sinr_{\textrm{dB},k} > \tau\}}}{K} 
\]
\end{comment}
